Optimal-transport-based metric for SMLM

We propose the use of Flat Metric to assess the performance of reconstruction methods for single-molecule localization microscopy (SMLM) in scenarios where the ground-truth is available. Flat Metric is intimately related to the concept of optimal transport between measures of different mass, providing solid mathematical foundations for SMLM evaluation and integrating both localization and detection performance. In this paper, we provide the foundations of Flat Metric and validate this measure by applying it to controlled synthetic examples and to data from the SMLM 2016 Challenge.

==> figs/UOT_results_example.tex <==
\def\radiusscale{.01}
\def\transportscale{2}
\def\scale{4.0}
\def\experiment{trial}
\def\radiusscale{.1}
\input{figs/UOT_results_template}
